Time Delays in Membrane Systems and Petri Nets

Timing aspects in formalisms with explicit resources and parallelism are investigated, and it is presented a formal link between timed membrane systems and timed Petri nets with localities. For both formalisms, timing does not increase the expressive power; however both timed membrane systems and timed Petri nets are more flexible in describing molecular phenomena where time is a critical resource. We establish a link between timed membrane systems and timed Petri nets with localities, and prove an operational correspondence between them.

==> eptcsdata.tex <==
\providecommand{\firstpage}{47}
\providecommand{\publicationstatus}{M. Massink and G. Norman (Eds.): 9th Workshop on\\ Quantitative Aspects of Programming Languages (QAPL 2011)\\
EPTCS 57, 2011, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.57.4}{10.4204/EPTCS.57.4}}

